The general theory of permutation equivarant neural networks and higher order graph variational encoders

Previous work on symmetric group equivariant neural networks generally only considered the case where the group acts by permuting the elements of a single vector. In this paper we derive formulae for general permutation equivariant layers, including the case where the layer acts on matrices by permuting their rows and columns simultaneously. This case arises naturally in graph learning and relation learning applications. As a specific case of higher order permutation equivariant networks, we present a second order graph variational encoder, and show that the latent distribution of equivariant generative models must be exchangeable. We demonstrate the efficacy of this architecture on the tasks of link prediction in citation graphs and molecular graph generation.

==> fig_mols_gen_20.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}%[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/large_mols_img_20_1.pdf}
        \caption{The only eight molecules with more than 10 atoms generated when using the KL Divergence term.}
    \end{subfigure}%
    \begin{subfigure}%[b]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/large_mols_img_20_0.pdf}
        \caption{A sampling of 12 molecules with more than 10 atoms generated without the KL Divergence term.}
    \end{subfigure}
    % \caption{Caption place holder}
\end{figure*}


==> link_prediction.tex <==
\subsection{Link prediction on citation graphs}
\label{sec:link_prediction}

 We demonstrate the ability of the SnNN models to learn meaningful latent embeddings on a link prediction task on popular citation network datasets Cora and Citeseer \citep{PSen2008}. In the training time, 15\% of the citation links (edges) have been removed while all node features are kept, the models are trained on an incomplete graph Laplacian constructed from the rest 85\% of the edges. From previously removed edges, we sample the same number of pairs of unconnected nodes (non-edges). We form the validation and test sets that contain 5\% and 10\% of edges with an equal amount of non-edges, respectively. Hyperparameters optimization (e.g. number of layers, dimension of the latent representation, etc.) is done on the validation set. \\ \\
 We compare our model SnNN against spectral clustering (SC) \citep{Tang2011}, deep walk (DW) \citep{Perozzi2014}, non-probabilistic graph autoencoder (GAE) and variational graph autoencoder (VGAE) \citep{kipf2016variational} on the ability to correctly classify edges and non-edges using two metrics: area under the ROC curve (AUC) and average precision (AP). Numerical results of SC, DW, GAE and VGAE and experimental settings are taken from \citep{kipf2016variational}. For SnNN, we initialize weights by Glorot initialization \cite{Glorot2010}. We train for 2,048 epochs using Adam optimization \cite{Kingma2015} with a starting learning rate of $0.01$. The number of layers range from 1 to 4. The size of latent representation is 64. \\ \\
Tables \ref{tbl:cora} and \ref{tbl:citeseer} show our numerical results in Cora and Citeseer datasets. SnNN outperforms all other baselines, especially VGAE with a considerable margin of 5\% in AUC and 2\% in AP.

\begin{table}
\caption{\label{tbl:cora} Cora link prediction results (AUC \& AP)}
\begin{center}
\begin{tabular}{||l | c | c ||}
	\hline
	Method & AUC & AP \\
	\hline\hline
	SC & 84.6 $\pm$ 0.01 & 88.5 $\pm$ 0.00 \\
	\hline
	DW & 83.1 $\pm$ 0.01 & 85.0 $\pm$ 0.00 \\
	\hline
	GAE & 91.0 $\pm$ 0.02 & 92.0 $\pm$ 0.03 \\
	\hline
	VGAE & 91.4 $\pm$ 0.01 & 92.6 $\pm$ 0.01 \\
	\hline
	\textbf{SnNN} & \textbf{96.1 $\pm$ 0.07} & \textbf{96.4 $\pm$ 0.06} \\
	\hline
\end{tabular}
\end{center}
\end{table}

\begin{table}
\caption{\label{tbl:citeseer} Citeseer link prediction results (AUC \& AP)}
\begin{center}
\begin{tabular}{||l | c | c ||}
	\hline
	Method & AUC & AP \\
	\hline\hline
	SC & 80.5 $\pm$ 0.01 & 85.0 $\pm$ 0.01 \\
	\hline
	DW & 80.5 $\pm$ 0.02 & 83.6 $\pm$ 0.01 \\
	\hline
	GAE & 89.5 $\pm$ 0.04 & 89.9 $\pm$ 0.05 \\
	\hline
	VGAE & 90.8 $\pm$ 0.02 & 92.0 $\pm$ 0.02 \\
	\hline
	\textbf{SnNN} & \textbf{95.3 $\pm$ 0.01} & \textbf{94.3 $\pm$ 0.01} \\
	\hline
\end{tabular}
\end{center}
\end{table}


==> molecular_generation.tex <==
\subsection{Molecular generation}
\label{sec:molecular-generation}


% We compare SnNN against ... in the task of molecular generation. 
To test the ability of the Sn-equivariant layers (defined in corollary \ref{coro: second order}) to build structured graphs, we apply them to molecular generation.
A key point of our work is that we incorporate no domain knowledge in our architecture:
any information about molecular structure is learned directly by the network.
This demonstrates the ability of networks using higher-order equivariant layers to learn more complex structures.

We build a variational autoencoder using the second-order equivariant activation described in section \ref{sec: vae}.
Both the encoder and the decoder have 4 layers of with 100 channel indices, followed by a ReLU nonlinearity.
Our prior consists of a \sm{\mathcal{N}\left(0,1\right)} distribution on a \sm{n \times 7} dimensional space, where $n$ is the number of nodes in the largest graph considered.
%(see section \ref{sec:latent}).
Consequently, the final layer of our encoder mixes down to 14 channels, 7 of which correspond to the means and 7 of which correspond to the variances in the approximate posterior $q_\phi$ of the variational autoencoder.
All models were trained and validated on ZINC dataset \citep{Sterling2015} using the testing split described in \citep{pmlr-v70-kusner17a}.
In table~\ref{tbl:zinc}, we report numerical results for two metrics: reconstruction accuracy of molecules in the test set, and validity of new molecules generated from the prior
and compare with other algorithms.
\begin{table}[t]
\caption{\label{tbl:zinc} ZINC results (reconstruction accuracy \& validity)}
\begin{center}
\begin{tabular}{||l | c | c ||}
	\hline
	Method & Accuracy & Validity \\ 
	\hline\hline
	CVAE & 44.6\% & 0.7\% \\
	\hline
	GVAE & 53.7\% & 7.2\% \\
	\hline
	SD-VAE & 76.2\% & 43.5\% \\
	\hline
	GraphVAE & - & 13.5\% \\
    \hline
	Atom-by-Atom LSTM & - & 89.2\% \\
	\hline
	JT-VAE & 76.7\% & 100.0\% \\
	\hline
	\textbf{SnNN} & \textbf{76.0\%} & \textbf{74\%} \\
	\hline
\end{tabular}
\end{center}
\end{table}
\ignore{
\begin{table}[t]
\caption{\label{tbl:qm9} QM9 results (reconstruction accuracy \& validity)}
\begin{tabular}{||l | c | c ||}
	\hline
	Method & Reconstruction accuracy & Validity \\
	\hline\hline
	\hline
\end{tabular}
\end{table}
}
Our results are comparable to other leading algorithms, having a similar reconstruction accuracy to Junction-Tree variational autoencoder (JT-VAE) \citep{DBLP:journals/corr/abs-1802-04364} and Syntax-Directed variational autoencoder (SD-VAE) \citep{DBLP:journals/corr/abs-1802-08786}. Both JT-VAE and the Atom-by-Atom LSTM \citep{DBLP:journals/corr/abs-1803-03324} construct more valid molecules.
However, we note that our algorithm requires considerably less domain knowledge than many of the other algorithms in \ref{tbl:zinc}.
The SD-VAE, Grammar VAE (GVAE) \citep{pmlr-v70-kusner17a}, and Character VAE (CVAE) \citep{Bombarelli2016} treat the task of molecular graph generation as text generation in Natural Language Processing by explicitly using the SMILES strings: structured representations of molecules that, in their construction, encode rules about chemical connectivity.
JT-VAE explicitly draws from a vocabulary of chemical structures and explicitly ensures that the output obeys known chemical rules.
In constrast, our model is given no knowledge of basic chemical principles such as valency, and must learn it by itself.

\input{../draft/fig-mols-gen.tex}

We next test the ability of the architecture to generate new molecules.  We sample 5000 IID normal vectors from the prior, and construct the corresponding graphs from the decoder.
We found that our model does not learn to construct construct a single, connected graph; consequently we take the largest connected component of the graph as our predicted molecule.
Indeed, this procedure biases our results towards small molecules: over 80 percent of the valid molecules we generate have 5 heavy atoms or less.
In figure \ref{fig:large_molecules} we give a sample of 16 generated molecules that are syntactically valid and have more than 10 atoms.

% Comparing with the molecules in the ZINC dataset, we observe that our network constructs many molecules that are sterically strained, with 3-atom and 4-atom rings.
% Real molecules are more likely to have rings with 5-8 atoms.  
% These patterns are clear examples of higher-order features, and we theorize that future work that uses higher-order forms of equivariance will improve on these aspects of predictions.
% However, we also note that our predictions have clear carbon-backbones

